Invertible Kernel PCA with Random Fourier Features

Kernel principal component analysis (kPCA) is a widely studied method to construct a low-dimensional data representation after a nonlinear transformation. The prevailing method to reconstruct the original input signal from kPCA -- an important task for denoising -- requires us to solve a supervised learning problem. In this paper, we present an alternative method where the reconstruction follows naturally from the compression step. We first approximate the kernel with random Fourier features. Then, we exploit the fact that the nonlinear transformation is invertible in a certain subdomain. Hence, the name \emph{invertible kernel PCA (ikPCA)}. We experiment with different data modalities and show that ikPCA performs similarly to kPCA with supervised reconstruction on denoising tasks, making it a strong alternative.

==> tikz/usps_pca_components_noise_3d_ikpca_app.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}

% Viridris colomap but shifted, see here for values https://matplotlib.org/3.1.1/tutorials/colors/colormap-manipulation.html
\pgfplotsset{colormap={mycolormap}{rgb(-500)=(0.267004,0.004874,0.329415) rgb(0)=(0.143343,0.522773,0.55629) rgb(1500)=(0.993248,0.906157,0.143936)}}


\begin{tikzpicture}[baseline]
    \pgfplotstableread[col sep=comma]{./data/usps/noise_3d.csv}{\datatableavg};
    \begin{axis}[
        width=0.9\linewidth,
        height=1.1\linewidth,
        title={ikPCA, $\log_{10}(\mathrm{MSE})$},
        %ylabel={principle components $\dimLatent$},
        xlabel={noise level $\sigma$},
        % xmin=0.3,
        % xmax=12,
        % ymin=3e-3,
        % ymax=1.5,
        view={0}{90},
        extra tick style={tickwidth=\pgfkeysvalueof{/pgfplots/minor tick length},},
        colorbar,
        colorbar style={width=2mm,
        	at={(1.1,0.5)},anchor=east,
        	ticklabel style={font=\scriptsize},
        },
        colormap name ={mycolormap},
    ]

        \addplot3 [surf, mesh/rows=18, shader=faceted] table[x=noise, y=pca_components, z=mse_ikpca_list_log10, col sep=comma] {\datatableavg}; % number of principle components = mesh/row



    \end{axis}
\end{tikzpicture}

==> tikz/usps_pca_components_noise_3d_kpca_app.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}

% Viridris colomap but shifted, see here for values https://matplotlib.org/3.1.1/tutorials/colors/colormap-manipulation.html
\pgfplotsset{colormap={mycolormap}{rgb(-500)=(0.267004,0.004874,0.329415) rgb(0)=(0.143343,0.522773,0.55629) rgb(1500)=(0.993248,0.906157,0.143936)}}


\begin{tikzpicture}[baseline]
    \pgfplotstableread[col sep=comma]{./data/usps/noise_3d.csv}{\datatableavg};
    \begin{axis}[
        width=0.9\linewidth,
        height=1.1\linewidth,
        title={kPCA+SL, $\log_{10}(\mathrm{MSE})$},
        %ylabel={principle components $\dimLatent$},
        xlabel={noise level $\sigma$},
        % xmin=0.3,
        % xmax=12,
        % ymin=3e-3,
        % ymax=1.5,
        view={0}{90},
        colorbar,
        extra tick style={tickwidth=\pgfkeysvalueof{/pgfplots/minor tick length},},
        colorbar style={width=2mm,
	        	at={(1.1,0.5)},anchor=east,
	        	ticklabel style={font=\scriptsize},
	        },
        colormap name ={mycolormap},
    ]

        \addplot3 [surf, mesh/rows=18, shader=faceted] table[x=noise, y=pca_components, z=mse_kpca_list_log10, col sep=comma] {\datatableavg}; % number of principle components = mesh/row



    \end{axis}
\end{tikzpicture}

==> tikz/usps_pca_components_noise_3d_pca_app.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}

% Viridris colomap but shifted, see here for values https://matplotlib.org/3.1.1/tutorials/colors/colormap-manipulation.html
\pgfplotsset{colormap={mycolormap}{rgb(-500)=(0.267004,0.004874,0.329415) rgb(0)=(0.143343,0.522773,0.55629) rgb(1500)=(0.993248,0.906157,0.143936)}}


\begin{tikzpicture}[baseline]
    \pgfplotstableread[col sep=comma]{./data/usps/noise_3d.csv}{\datatableavg};
    \begin{axis}[
        width=0.9\linewidth,
        height=1.1\linewidth,
        title={PCA, $\log_{10}(\mathrm{MSE})$},
        ylabel={principle components $\dimLatent$},
        xlabel={noise level $\sigma$},
        % xmin=0.3,
        % xmax=12,
        % ymin=3e-3,
        % ymax=1.5,
        view={0}{90},
        extra tick style={tickwidth=\pgfkeysvalueof{/pgfplots/minor tick length},},
        colorbar,
        colorbar style={width=2mm,
        				at={(1.1,0.5)},anchor=east,
        				ticklabel style={font=\scriptsize},
        				},
        colormap name ={mycolormap},
    ]

        \addplot3 [surf, mesh/rows=18, shader=faceted] table[x=noise, y=pca_components, z=mse_pca_list_log10, col sep=comma] {\datatableavg}; % number of principle components = mesh/row



    \end{axis}
\end{tikzpicture}
